Semisimplicity and Reduction of p-adic Representations of Topological Monoids

We give a criterion of the semisimplicity of a p-adic unitary representation of a topological monoid by the reduction of the associated operator algebra.

==> idempotents.tex <==
\section{Idempotents}
\label{Idempotents}



In this section, let $k$ denote a local field. For a ring $A$, an $e \in A$ is said to be an {\it idempotent} if $e^2 = e$.



\input{li}

